Inferring the Rotation Period Distribution of Stars from their Projected Rotation Velocities and Radii: Application to late-F/early-G Kepler Stars

While stellar rotation periods $P_\mathrm{rot}$ may be measured from broadband photometry, the photometric modulation becomes harder to detect for slower rotators, which could bias measurements of the long-period tail of the $P_\mathrm{rot}$ distribution. Alternatively, the $P_\mathrm{rot}$ distribution of stars can be inferred from their projected rotation velocities $v\sin i$ and radii $R$, without being biased against photometrically quiet stars. We solve this inference problem using a hierarchical Bayesian framework, which (i) is applicable to heteroscedastic measurements of $v\sin i$ and $R$ with non-Gaussian uncertainties and (ii) does not require a simple parametric form for the true $P_\mathrm{rot}$ distribution. We test the method on simulated data sets and show that the true $P_\mathrm{rot}$ distribution can be recovered from $\gtrsim 100$ sets of $v\sin i$ and $R$ measured with precisions of $1\,\mathrm{km/s}$ and $4\%$, respectively, unless the true distribution includes sharp discontinuities. We apply the method to a sample of 144 late-F/early-G dwarfs in the Kepler field with $v\sin i$ measured from Keck/HIRES spectra, and find that the typical rotation periods of these stars are similar to the photometric periods measured from Kepler light curves: we do not find a large population of slow rotators that are missed in the photometric sample, although we find evidence that the photometric sample is biased for young, rapidly-rotating stars. Our results also agree with asteroseismic measurements of $P_\mathrm{rot}$ for Kepler stars with similar ages and effective temperatures, and show that $\approx 1.1\,M_\odot$ stars beyond the middle of their main-sequence lifetimes rotate faster than predicted by standard magnetic braking laws.

==> table4_full.tex <==
\begin{table}
    \centering
    \caption{Information on the 144 stars used for the main analysis. Only first five entries are shown. Full table is available online. Other parameters are also available from \url{https://github.com/kemasuda/prot_from_vsini}.}
    \label{tab:catalog}
    \begin{tabular}{cccc}
    \hline\hline
    KIC & $T_{\rm eff}$ (K) & $v\sin i$ (km/s) & radius ($R_\odot$) \\
    \hline 
2158850 & 6038 & 2.7 & $1.15\pm0.05$\\
2998253 & 6291 & 9.2 & $1.45\pm0.06$\\
3338777 & 5993 & 6.9 & $2.37\pm0.10$\\
3831297 & 6111 & 3.6 & $1.13\pm0.04$\\
3936993 & 6176 & 7.9 & $1.85\pm0.07$\\
3952307 & 6102 & 4.3 & $2.17\pm0.09$\\
3967859 & 5948 & 1.8 & $1.27\pm0.05$\\
4039966 & 6221 & 9.6 & $1.11\pm0.04$\\
4147444 & 6305 & 14.3 & $1.18\pm0.04$\\
4346201 & 6103 & 5.1 & $2.05\pm0.09$\\
4475010 & 6642 & 33.1 & $1.99\pm0.10$\\
4484238 & 6169 & 7.3 & $1.42\pm0.06$\\
4645245 & 6119 & 5.0 & $1.10\pm0.04$\\
4753390 & 6378 & 11.0 & $1.93\pm0.14$\\
4755204 & 5878 & 3.2 & $1.61\pm0.07$\\
5094944 & 6442 & 13.7 & $1.35\pm0.05$\\
5183581 & 6316 & 10.8 & $2.11\pm0.08$\\
5184384 & 6072 & 6.0 & $1.96\pm0.10$\\
5357446 & 6218 & 15.4 & $1.15\pm0.05$\\
5446518 & 6350 & 28.2 & $1.25\pm0.05$\\
5468089 & 6210 & 8.9 & $2.00\pm0.08$\\
5510904 & 6431 & 14.7 & $1.38\pm0.05$\\
5514383 & 6209 & 7.5 & $1.20\pm0.05$\\
5531145 & 6517 & 17.7 & $2.24\pm0.09$\\
5724853 & 5913 & 2.9 & $1.09\pm0.04$\\
5803208 & 6439 & 14.1 & $1.52\pm0.06$\\
5856836 & 6287 & 7.6 & $1.40\pm0.05$\\
5865892 & 6406 & 7.7 & $1.45\pm0.06$\\
5866724 & 6265 & 9.1 & $1.42\pm0.05$\\
5871558 & 6155 & 5.8 & $2.25\pm0.09$\\
5899165 & 6104 & 3.7 & $1.10\pm0.04$\\
6280366 & 6302 & 7.2 & $1.44\pm0.06$\\
6285677 & 6165 & 8.6 & $1.21\pm0.05$\\
6314137 & 6390 & 9.5 & $1.36\pm0.05$\\
6359801 & 6635 & 26.5 & $1.80\pm0.07$\\
6364123 & 6113 & 4.0 & $1.75\pm0.07$\\
6425358 & 6166 & 4.8 & $1.35\pm0.05$\\
6438107 & 6084 & 5.5 & $2.12\pm0.08$\\
6547806 & 6268 & 13.6 & $3.51\pm0.17$\\
6680045 & 6160 & 5.0 & $1.21\pm0.05$\\
6689943 & 6069 & 5.9 & $1.59\pm0.06$\\
6777975 & 6325 & 12.6 & $1.18\pm0.04$\\
7050604 & 6298 & 10.5 & $1.19\pm0.04$\\
7094508 & 6244 & 7.0 & $2.34\pm0.09$\\
7206837 & 6429 & 8.7 & $1.61\pm0.06$\\
7260381 & 6113 & 4.2 & $1.22\pm0.05$\\
7383120 & 6089 & 3.5 & $1.44\pm0.06$\\
7422905 & 5992 & 1.7 & $1.06\pm0.04$\\
7434909 & 5975 & 2.3 & $1.21\pm0.05$\\
7447105 & 6316 & 18.8 & $1.17\pm0.04$\\
7465902 & 6171 & 6.5 & $1.43\pm0.06$\\
7670943 & 6372 & 11.8 & $1.41\pm0.05$\\
7671716 & 6352 & 35.6 & $1.25\pm0.05$\\
7811344 & 6263 & 9.1 & $1.39\pm0.05$\\
7880676 & 6180 & 5.3 & $2.24\pm0.09$\\
7955048 & 6421 & 12.1 & $1.22\pm0.05$\\
8013078 & 6090 & 3.2 & $1.51\pm0.06$\\
8017790 & 6041 & 4.1 & $1.13\pm0.04$\\
8025283 & 5919 & 2.6 & $1.02\pm0.04$\\
8043167 & 6282 & 15.1 & $1.12\pm0.04$\\
8077525 & 6236 & 3.5 & $1.23\pm0.05$\\
8112746 & 6125 & 3.5 & $1.32\pm0.05$\\
8228742 & 6059 & 4.3 & $1.86\pm0.07$\\
8265838 & 6331 & 8.9 & $2.36\pm0.11$\\
8289241 & 6245 & 7.0 & $1.37\pm0.05$\\
8391021 & 6249 & 6.5 & $1.48\pm0.06$\\
8410157 & 5934 & 4.9 & $1.38\pm0.05$\\
8420801 & 6225 & 7.2 & $1.78\pm0.07$\\
8493800 & 6033 & 5.7 & $1.48\pm0.06$\\
8494872 & 6081 & 4.9 & $1.17\pm0.05$\\
8623058 & 6243 & 5.5 & $1.37\pm0.05$\\
8650186 & 6172 & 4.9 & $1.37\pm0.05$\\
8696343 & 5988 & 4.5 & $1.28\pm0.05$\\
8717023 & 6168 & 4.9 & $1.26\pm0.05$\\
9007356 & 5960 & 3.6 & $1.67\pm0.07$\\
9157245 & 5969 & 4.1 & $1.30\pm0.05$\\
9225600 & 6244 & 6.2 & $1.85\pm0.07$\\
9225997 & 5984 & 2.9 & $1.07\pm0.04$\\
9273544 & 6053 & 3.6 & $1.58\pm0.06$\\
9289275 & 6086 & 6.9 & $1.80\pm0.07$\\
9329766 & 5966 & 3.0 & $1.01\pm0.04$\\
9347707 & 6491 & 18.2 & $1.41\pm0.05$\\
9390670 & 6406 & 15.9 & $1.77\pm0.08$\\
9402223 & 6381 & 12.6 & $2.67\pm0.10$\\
9402649 & 6129 & 5.5 & $1.45\pm0.06$\\
9468847 & 5964 & 6.6 & $1.80\pm0.07$\\
9529969 & 5952 & 3.0 & $1.52\pm0.06$\\
9579208 & 6248 & 7.8 & $1.81\pm0.07$\\
9592705 & 6196 & 7.9 & $2.16\pm0.09$\\
9613220 & 6091 & 2.9 & $1.51\pm0.06$\\
9634952 & 6601 & 15.6 & $1.37\pm0.05$\\
9644337 & 6294 & 8.9 & $1.49\pm0.06$\\
9651253 & 6129 & 4.8 & $1.14\pm0.04$\\
9664404 & 5950 & 3.5 & $1.25\pm0.05$\\
9754284 & 6048 & 3.9 & $1.62\pm0.06$\\
9777798 & 5945 & 6.0 & $1.97\pm0.08$\\
9814780 & 6076 & 3.4 & $1.10\pm0.04$\\
9837454 & 5948 & 4.0 & $2.23\pm0.09$\\
9898249 & 6441 & 13.7 & $1.49\pm0.06$\\
9912680 & 6066 & 5.0 & $2.01\pm0.08$\\
10006140 & 6146 & 4.4 & $1.18\pm0.05$\\
10016032 & 6298 & 7.0 & $1.17\pm0.04$\\
10016239 & 6384 & 13.0 & $1.32\pm0.05$\\
10024648 & 6246 & 9.2 & $2.01\pm0.08$\\
10025841 & 5996 & 4.0 & $1.61\pm0.06$\\
10079226 & 5974 & 3.5 & $1.17\pm0.05$\\
10097040 & 6245 & 6.2 & $1.37\pm0.05$\\
10322381 & 6149 & 4.5 & $1.39\pm0.05$\\
10351834 & 6327 & 24.4 & $1.17\pm0.04$\\
10418344 & 6486 & 18.3 & $2.55\pm0.13$\\
10651962 & 6185 & 5.1 & $1.29\pm0.05$\\
10732086 & 6173 & 10.2 & $1.11\pm0.04$\\
10813492 & 6071 & 6.2 & $1.47\pm0.06$\\
10813660 & 6138 & 5.3 & $1.44\pm0.06$\\
10907438 & 6122 & 5.1 & $2.26\pm0.09$\\
10974969 & 6000 & 7.8 & $2.83\pm0.11$\\
10988876 & 6133 & 2.6 & $1.17\pm0.05$\\
11025641 & 6135 & 4.0 & $2.13\pm0.09$\\
11136719 & 6536 & 16.3 & $1.89\pm0.07$\\
11197632 & 6083 & 3.7 & $1.17\pm0.05$\\
11283797 & 5979 & 4.4 & $1.04\pm0.04$\\
11362858 & 6367 & 10.9 & $1.17\pm0.04$\\
11389437 & 6060 & 5.7 & $1.74\pm0.07$\\
11444160 & 6149 & 6.4 & $1.17\pm0.05$\\
11453915 & 6359 & 8.0 & $1.24\pm0.05$\\
11467550 & 6111 & 7.1 & $2.02\pm0.08$\\
11512820 & 6244 & 2.6 & $1.08\pm0.04$\\
11599875 & 6118 & 9.3 & $1.68\pm0.07$\\
11654380 & 5972 & 5.4 & $1.57\pm0.06$\\
11710285 & 6351 & 6.9 & $1.50\pm0.06$\\
11754352 & 6208 & 4.9 & $1.47\pm0.06$\\
11763874 & 6023 & 4.7 & $1.42\pm0.06$\\
11807274 & 6247 & 10.3 & $1.59\pm0.06$\\
11870319 & 6124 & 5.1 & $1.45\pm0.07$\\
11910501 & 6193 & 9.1 & $1.66\pm0.07$\\
12006631 & 6143 & 3.1 & $1.15\pm0.04$\\
12009504 & 6107 & 6.7 & $1.46\pm0.06$\\
12058453 & 6010 & 4.0 & $1.33\pm0.05$\\
12069127 & 6267 & 3.8 & $2.35\pm0.09$\\
12072958 & 5978 & 9.1 & $0.97\pm0.04$\\
12117868 & 5967 & 3.6 & $1.32\pm0.05$\\
12265063 & 5913 & 3.9 & $1.67\pm0.07$\\
12555240 & 6120 & 2.2 & $1.22\pm0.05$\\
12785394 & 6527 & 17.7 & $1.43\pm0.05$\\
    \hline
    \end{tabular}
\end{table}
